Finite-State Dimension and Lossy Decompressors

This paper examines information-theoretic questions regarding the difficulty of compressing data versus the difficulty of decompressing data and the role that information loss plays in this interaction. Finite-state compression and decompression are shown to be of equivalent difficulty, even when the decompressors are allowed to be lossy. Inspired by Kolmogorov complexity, this paper defines the optimal *decompression *ratio achievable on an infinite sequence by finite-state decompressors (that is, finite-state transducers outputting the sequence in question). It is shown that the optimal compression ratio achievable on a sequence S by any *information lossless* finite state compressor, known as the finite-state dimension of S, is equal to the optimal decompression ratio achievable on S by any finite-state decompressor. This result implies a new decompression characterization of finite-state dimension in terms of lossy finite-state transducers.

==> bigpage-corr-graphicx.tex <==
% This is a file needed to make the pages not look bad after going
% through CoRR's automatic compilation that normally destroys margins.
% Also, it corrects whatever graphics does.

\oddsidemargin  0.0in
\evensidemargin 0.0in
\textwidth      6.3in
\headheight     0.0in
\topmargin      0.1in
\textheight     8.5in


